Reachability relations of timed pushdown automata

Timed pushdown automata (TPDA) are an expressive formalism combining recursion with a rich logic of timing constraints. We prove that reachability relations of TPDA are expressible in linear arithmetic, a rich logic generalising Presburger arithmetic and rational arithmetic. The main technical ingredients are a novel quantifier elimination result for clock constraints (used to simplify the syntax of TPDA transitions), the use of clock difference relations to express reachability relations of the fractional clock values, and an application of Parikh's theorem to reconstruct the integral clock values.

==> 1-ta.tex <==

% !TEX root = main.tex

\section{Timed automata with one clock}
\label{sec:1-TA}

In this section we show that, in the case of only one clock,
we can represent the reachability relation with a hybrid formula of polynomial size.
%
In a one clock \TA, all constraints are already non-diagonal.
In the rest of the section, we construct an \NFA $B$
and construct the reachability relation of $A$ from the Parikh image of $B$.
%
The size of $B$ will be polynomial in the size of $A$.

\paragraph{Interval abstraction}
%
We replace the integer value of the clock $x$ by its interval.
Let $0 = k_0 < k_1 < \cdots < k_n < k_{n+1} = \infty$
be all constants appearing in clock constraints of $A$ of the form $x \sim k_i$,
and let the set of intervals be the following totally ordered set:
%
\begin{align*} 
	\Lambda = \set{ \set {k_0} < (k_0, k_1) < \set {k_1} < \cdots < (k_{n-1}, k_n) < \set {k_n} < (k_n, k_{n+1})}.
\end{align*}
%
%For $\lambda_i \in \set{\set {k_i}, (k_i, k_{i+1})}$ and $\lambda_j \in \set{\set {k_j}, (k_j, k_{j+1})}$
%with $\lambda_j \geq \lambda_i$, let $\lambda_j - \lambda_i$ be defined as $k_j - k_i$.
%
Clearly, we can resolve any constraint $\varphi$ of $A$
by looking at the current interval $\lambda \in \Lambda$:
$\mu \models \varphi$ iff $\nu \models \varphi$ for every $\nu \in \lambda_\mu$,
where $\lambda_\mu$ is the unique interval in $\Lambda$ \st $\mu(x)$ belongs to it.
%
We write $\lambda \models \varphi$ whenever $\mu \models \varphi$ for some $\mu \in \lambda$,
whose choice does not matter by the previous observation.
%
Let $\varphi_\lambda$ be the \emph{characteristic constraint} of the interval $\lambda$.
%
For a constraint $\varphi$,
let $\restrict \varphi \lambda$ be $\varphi$
where every constraint $\floor \x \leq k$ %or modulo constraint $\floor \x \eqv M k$
or $\fract x \sim 0$
is uniquely resolved to be $\true$ or $\false$ by looking at $\lambda$.

\paragraph{Region abstraction}
%
We introduce an extra clock $x_0$ which is never reset and never appears in any constraint.
It is used only to keep track of the fractional elapse of time,
and its relationship with the fractional part of clock $x$.
%
%A \emph{region} $r$ is a set of clock valuations
We distinguish the following 6 regions relating the fractional parts of $x_0$ and $x$:
%
\begin{align*}
	\xi_0 \;&\equiv\; 0 = \fract {x_0} = \fract x < 1
	& \xi_1 \;&\equiv\; 0 = \fract {x_0} < \fract x < 1 \\
	\xi_2 \;&\equiv\; 0 < \fract {x_0} = \fract x < 1
	&\xi_3 \;&\equiv\; 0 < \fract {x_0} < \fract x < 1 \\
	\xi_4 \;&\equiv\; 0 = \fract {x} < \fract {x_0} < 1
	&\xi_5 \;&\equiv\; 0 < \fract {x} < \fract {x_0} < 1.
\end{align*}
%
Let $\Xi = \set {\xi_0, \dots, \xi_5}$.
When time elapses, and when $x$ is reset,
we move deterministically from region to region according to the following rules:
%
\begin{align*}
	&\xi_0 \goesto {\elapse} \xi_2 \goesto {\elapse} \xi_0
	&&\xi_1 \goesto {\elapse} \xi_3 \goesto {\elapse} \xi_4 \goesto {\elapse} \xi_5 \goesto {\elapse} \xi_1 \\
	%
	&\xi_0, \xi_1 \goesto{\resetop{\x}} \xi_0
	&&\xi_2, \xi_3, \xi_4, \xi_5 \goesto{\resetop{\x}} \xi_4.
\end{align*}

\paragraph{The construction}
%
Let $A = (\Sigma, L, \X, \Delta)$ be a \TA
and we build an \NFA $B = (\Sigma', L', \to)$
where $\Sigma' \supseteq \Sigma$ is an extended alphabet
containing a tick symbol $\tick \lambda \not\in\Sigma$ for every interval $\lambda \in \Lambda$
%$k = k_j - k_i \geq 0$,
%measuring the discrete time elapse of $k$ time units,
%and a single symbol $\delta \not\in\Sigma$,
%measuring a fractional time elapse of any amount in $(0, 1)$,
and $L' = L \times \Lambda \times \Xi \times \set{\bot, \topbot, \top}$ %\Xi_\bot
is a set of states of the form $(p, \lambda, \xi, f)$,
where $p \in L$ is a control location of $A$,
$\lambda \in \Lambda $ is an interval,
$\xi \in \Xi$ is a region,
$f \in \set{\bot, \topbot, \top}$ is a flag determining whether
a) the clock $x$ must still be reset (if $r = \bot$),
b) the clock $x$ will not be reset anymore (if $r = \topbot$),
c) no time elapse is allowed anymore (if $r = \top$),
%where $r$ is a flag determining whether the clock $x$ can still be reset (if $r = \bot$),
%or not (if $r \neq \bot$, in which case $r$ records the region of the last time $x$ was reset),
satisfying the following constraint: if $\lambda = \set {k_i}$, then $\xi \in \set {\xi_0, \xi_4}$.
Transitions are defined as follows.
%
Every transition $\trule p \op q \in \Delta$ generates one or more transitions in $B$ depending on $\op$.
%Assume that the initial control location of $A'$ is $\tuple {p, \lambda, \ZZ}$.
%
If $\op = \readop a$, then there are transitions of the form
$(p, \lambda, \xi, f) \goesto a (q, \lambda, \xi, f)$.
If $\op = \testop \varphi$, there there are all transitions of the form
$(p, \lambda, \xi, f) \goesto \varepsilon (q, \lambda, \xi, f)$ whenever $(\lambda, \xi) \models \varphi$.
%
An operation $\op = \resetop \x$ is only allowed in states where $r = \bot$:
%
$$(p, \lambda, \xi, \bot) \goesto {\tick \lambda} (q, \set 0, \xi', f'),$$
%
for the unique region $\xi'$ \st $\xi \goesto {\resetop x} \xi'$,
and for $r' = \bot$ if the automaton guesses there will be more resets in the future,
or $r' \in \set {\topbot, \top}$ in the opposite case.
%
If $\op = \elapse$, then we have transitions of the form
%
\begin{align*}
	(p, \lambda_i, \xi, f) &\goesto \varepsilon (q, \lambda_j, \xi', f),
\end{align*}
%
for every $\lambda_i \leq \lambda_j$, $\xi \goestostar \elapse \xi'$,
$f \in \set{\top, \topbot}$,
and $f' \in \set{ f, \top}$.
%
Finally, after the last reset the automaton also guesses the last time elapse,
and emits a final tick $\tick \lambda$:
%
\begin{align*}
	(p, \lambda, \xi, \topbot) &\goesto {\tick \lambda} (q, \lambda, \xi, \top),
\end{align*}
% \st the two tuples above are states of $B$.

\paragraph{Construction of the reachability relation of $A$}

For a set of finite words $L \subseteq (\Sigma')^*$,
let $\varphi_L(\# \bartick)$ be a formula of existential Presburger arithmetic of polynomial size
with a free variable $\#\tick \lambda$ for every interval $\lambda \in \Lambda$.
%
The total amount of integer time elapsed
%, depending on the initial $\xi$ and final region $\xi'$,
can be computed as follows:
%
\begin{align*}
	\tilde\varphi_{L} (\floor t) \; &\equiv\;
		\exists \# \bartick \st \varphi_L(\bartick) \wedge
		\exists \bar k \st \bigwedge_{\lambda \in \Lambda} (k_\lambda \in \#\tick \lambda \cdot \lambda) \wedge
		\floor t = \ignore{\delta_{\xi \xi'}} \sum_{\lambda \in \Lambda} k_\lambda. %, \textrm { where }
%	\delta_{\xi \xi'} \; &= \;
%		\left\{\begin{array}{ll}
%			0 & \\
%			1 & 
%		\end{array}\right.
\end{align*}

%
%Let $L(
%

Let $c$ be of the form $c = (p, \lambda, \xi, f)$ with $f \in \set{\bot, \topbot}$,
and $d$ of the form $d = (q, \lambda', \xi', \top)$:
%
\begin{align*}
	\varphi_\bot(x, t, x') \; &\equiv\;
		\true,
	\\
	\varphi_{\topbot}(x, t, x') \; &\equiv\;
		\floor {x' - x} = \floor t \wedge \fract {x' - x} = \fract t,
	\\
	\varphi_{cd}(x, t, x') \; &\equiv \;
		\floor x \in \lambda \wedge
		\floor {x'} \in \lambda' \wedge
		\xi(\fract t, \fract x) \wedge
		\xi'(\fract {t'}, \fract {x'}) \wedge
		\tilde\varphi_{L_{cd}}(\floor t) \wedge
		\varphi_f(x, t, x'),
	\\
	\varphi_{pq}(x, t, x') \; &\equiv \;
		\bigvee \setof {\varphi_{cd}(x, t, x')} {c = (p, \lambda, \xi, f), d = (q, \lambda', \xi', f')}.
\end{align*}
%
%The existential quantifiers above can be eliminated by appealing to quantifier elimination for Presburger logic.

==> reachset.tex <==
% !TEX root = main.tex

\subsection{Reduction to the reachability set}

\ilorenzo{Not clear how to use this observation in the context of \TPDA, where the reachability relation is a more natural object of study.}

In this section we show that computing the reachability relation $\reach{} {pq}$
effectively reduces to computing the reachability set $\ReachSet {pq}$.
%
Let $A$ be a \TPDA with set of clocks $\X$.
%
The idea is to introduce for each clock $\x \in \X$ a copy $\underline\x \in \underline \X$ thereof
s.t.~1) initially $\underline \x = \x$, and 2) $\underline \x$ is never reset.
We assume also the existence of a clock $\x_0 \in \X$ which is initially $0$ and is never reset.
%
Let $B$ be the resulting \TPDA over clocks $\Y = \X \cup \underline \X$.
%
If $\mu \reach w {pq} \nu$ in $B$, then,
since the copy clock $\underline\x$ is never reset, we have the following relationship
between the initial value of $\x$ and the final values of its copy $\underline \x$ and $\x_0$:
%
\begin{align*}
    \mu(\x) = \nu (\underline \x) - \nu(\x_0).
\end{align*}
%
This simple relationship allows us to reconstruct the reachability relation of $\A$
from the reachability set of $\B$.
%
Let $\varphi_{pq}(\bar \x', \bar {\underline \x}')$ be a \LA formula
expressing the reachability set $\ReachSet {pq}^B$ of $B$,
where $\bar \x'$ represents the final value of the original clocks of $A$
and $\bar {\underline \x}'$ for the copies thereof.
%
The reachability relation $\reach {} {pq}$ of $A$ is expressed by the \LA formula
%
\begin{align*}
    \psi_{pq}(\bar \x, \bar \x') \;\equiv\; \exists \bar {\underline \x}' \st \bar \x = \bar {\underline \x}' - \x_0' \wedge \varphi_{pq}(\bar \x', \bar {\underline \x}').
\end{align*}

==> ta.tex <==

% !TEX root = main.tex

\section{Timed automata}
\label{sec:TA}

\paragraph{The model.}

A \emph{timed automaton} (\TA) is a tuple
%
$\P = \tuple {\Sigma, L, \X, \Delta}$
%
where
$\Sigma$ is a finite input alphabet,
$L$ is a finite set of control locations,
$\X$ is a finite set of \emph{clocks},
and $\Delta$ is a set of transition rules of the form
$\trule p \op q$ with $p, q \in L$ control locations,
where $\op$ determines the type of transition:
%
\begin{itemize}
\item \emph{time elapse} $\op = \elapse$,
%
\item \emph{input} $\op = \readop a$ with $a \in \Sigma_\varepsilon := \Sigma \cup \{\varepsilon\}$ an input letter,
%
\item \emph{test} $\op = \testop \varphi$ a \emph{transition constraint} over clocks $\X$, and
%
\item \emph{reset} $\op = \resetop \Y$ with $\Y \subseteq \X$ a set of clocks to be reset.
%
\end{itemize}
%
Throughout the paper, let $\x_0$ be a control clock that is never reset
(and thus measures the total elapsed time).

\begin{remark}[Complexity]
	For complexity estimations, we assume that constraints are conjunctions of atomic constraints,
	that constants therein are encoded in binary,
	that $M$ is the maximal constant,
	and that all modular constraints use the same modulus $M$.
\end{remark}

\begin{remark}[Time elapse]
	The standard semantics of timed automata where time can elapse freely in every control location
	is simulated by adding explicit time elapse transitions
	$\trule{p}{\elapse}{q}$ for suitable locations $\ell$.
	%
	Our explicit modelling of the elapse of time will simplify the following constructions.
  % constructions in Sec.~\ref{sec:fractional}.
\end{remark}

\paragraph{Semantics.}
%
\ignore{
A \emph{configuration} is a pair $\tuple{p, \mu} \in L \times \Qgeq^\X$
where $p$ is a control location and $\mu$ is a clock valuation.
%
Let $\tuple{p, \mu}, \tuple{q, \nu}$ be two configurations.
%
For every input symbol $a \in \Sigma_\varepsilon$
and rule $\trule p \op q \in \Delta$,
we have a transition
%
\begin{gather*}
  \tuple{p, \mu} \goestoop a \op \tuple{q, \nu}
\end{gather*}
%
whenever one of the following holds:
%
\begin{itemize}
  %
  \item%[\bf (elapse)]
  $\op = \elapse$,
  $a = \varepsilon$, and there exists $\delta \geq 0$ \st $\nu = \mu + \delta$.
  %
  \item%[\bf (input)]
  $\op = \readop a$ and $\nu = \mu$.
  %
  \item%[\bf (test)]
  $\op = \testop \varphi$, $a = \varepsilon$, $\mu \models \varphi$, and $\nu = \mu$.
  %
  \item%[\bf (reset)]
  $\op = \resetop \Y$, $a = \varepsilon$, and $\nu = \mu[\Y \mapsto 0]$.
  %
\end{itemize}
%
We simply write $\goesto a$ when $\goestoop a \op$ holds for some $\op$,
and we extend the one-step transition relation $\goesto a$
to sequences $w \in \Sigma^*$ as $\goesto w$ in the natural way.
}
%
The \emph{reachability relation} of a \TA
is the family of relations %$\set{\reach {} {pq}}_{p, q \in Q}$
%
$$\reach {} {pq} \ \subseteq\ \Q^\X \times \Sigma^* \times \Q^\X, $$
%
one for each pair of control locations $p, q \in Q$,
\st each $\reach {} {pq}$ is the least relation
satisfying the following rules,
where $p, q, r \in Q$,
$\mu, \nu, \rho : \Q^\X$,
and $w, u, v \in \Sigma^*$:
%
\begin{align}
  \label{eq:reachrel:A}
  &\textrm{\em (input)} &&
    \frac{}{\mu \reach a {pq} \mu}
       \qquad &&\textrm{ if } \exists \trule p {\readop a} q \in \Delta \\[2ex]
  \label{eq:reachrel:B}
  &\textrm{\em (test)} &&
  \frac{}{\mu \reach \varepsilon {pq} \mu}
     \qquad &&\textrm{ if } \exists \trule p {\testop \varphi} q \in \Delta \st \mu \models \varphi \\[2ex]
  \label{eq:reachrel:C}
  &\textrm{\em (reset)} &&
  \frac{}{\mu \reach \varepsilon {pq} \mu [\Y \mapsto 0]}
     \qquad &&\textrm{ if } \exists \trule p {\resetop \Y} q \in \Delta \\[2ex]
  \label{eq:reachrel:D}
     &\textrm{\em (elapse)} &&
    \frac{}{\mu \reach \varepsilon {pq} \nu}
       \qquad &&\textrm{ if } \exists \trule p \elapse q \in \Delta, \delta \geq 0 \st \nu = \mu + \delta \\[2ex]
    \label{eq:reachrel:E}
 &\textrm{\em (transitivity)} &&
    \frac{\mu \reach u {pr} \rho \quad \rho \reach v {rq} \nu}{\mu \reach {uv} {pq} \nu}.
\end{align}

\subsection{Main result}

An \emph{regular atom} is a pair $(L, \varphi)$ where $L$ is a regular language
and $\varphi$ is a formula of hybrid linear arithmetic.
%
%For two atoms $(L, \varphi), (M, \psi)$,
%let $(L, \varphi)\cdot(M, \psi) = (L \cdot M, \varphi \circ \psi)$.
%and $(L, \varphi)^* = (L^*, \varphi^*)$.
%
The semantics $\sem{L, \varphi} \subseteq \Q^\X \times \Sigma^* \times \Q^\X$ of an atom
is the set of triples $(\mu, w, \nu)$ s.t.~$(\mu, \nu) \models \varphi$
and $w \in L$.
%
% runs $\pi = (p_0, \mu_0) \goesto {a_1} \cdots \goesto {a_n} (p_n, \mu_n)$
%s.t.~$a_1 \cdots a_n \in L$ and $\mu_0, \mu_n \models \varphi$.
%
A \emph{regular semiatom} is a finite sum of regular atoms $\alpha = (L_1, \varphi_1) + \cdots + (L_n, \varphi_n)$
(i.e., disjunctive normal form)
where we assume w.l.o.g.~that each $\varphi_i$'s occurs at most once up to logical equivalence;
%(since $\sem{(L, \varphi) + (M, \varphi)} = \sem{L \cup M, \varphi}$)
the semantics of a semiatom is the union of the semantics of its atoms.
%
We prove the following expressibility result.

\begin{theorem}
  The \TA reachability relation is expressible as a regular semiatom.
\end{theorem}

The construction is in two steps.
%
In the first step, we remove integral and modular constraints and obtain a fractional \TA.
The relationship between the initial and final integral values of clocks
is encoded in the recognised language.
%
In the second step, the reachability relation of a fractional \TA is built by a simple reachability construction,
relying on the fact that the logic of fractional constraints has quantifier elimination and finitely many regions.

\subsection{Step 1: From \TA to fractional \TA}
\label{sec:to:fractional:TA}

A \TA is \emph{fractional} if it has only fractional constraints.
%
By using a standard construction,
we preliminarily convert diagonal integral and modulo constraints
to their non-diagonal counterparts.

\paragraph{Unary abstraction.}
%
We replace the integer value of clocks by their unary abstraction.
%
Let $M \in \N$.
Valuations $\mu, \nu \in \Qgeq^X$ are \emph{$M$-unary equivalent}
%written $\mu \approx_M \nu$,
if, for every clock $\x \in \X$,
$\floor {\mu(\x)} \eqv M \floor{\nu(\x)}$ and $\floor{\mu(\x)} \leq M \iff \floor{\nu(\x)} \leq M$.
%
Let $\Lambda_M$ be the (finite) set of $M$-unary equivalence classes of clock valuations.
%
%For $\lambda \in \Lambda_M$ we abuse notation and write $\lambda(\x)$ to indicate $\mu(\x)$ for some $\mu\in\lambda$,
%where the choice of representative $\mu$ does not matter.
%
We write $\lambda[\Y \mapsto 0]$ for the equivalence class of
$\nu[\Y \mapsto 0]$
%
%and we write $\lambda[\x \mapsto \x + 1]$ for the equivalence class of
%$\nu[\x \mapsto \nu(\x)+1]$,
for some $\nu\in\lambda$ (whose choice is irrelevant).
%
Let $\varphi_\lambda$ be the \emph{characteristic formula} of the unary class $\lambda$,
which is in fact a constraint of the form
%
\begin{align}
 \varphi_\lambda(\vec \x) \equiv \bigwedge_{\x \in \X} \floor \x \eqv M \lambda(\x) \wedge (\floor \x < M \iff \lambda(\x) < M),
\end{align}
where $\lambda(\x)$ denotes $\nu(\x)$ for some $\nu\in\lambda$
(whose choice is irrelevant).
%say that clocks belong to $\lambda$.
%
For a constraint $\varphi$,
let $\restrict \varphi \lambda$ be $\varphi$
where every non-diagonal integer $\floor \x \leq k$ or modulo constraint $\floor \x \eqv M k$
is uniquely resolved to be $\true$ or $\false$ by looking at $\lambda$.

\paragraph{The construction.}
%
%Recall the structure of fractional values $\AIc = (\I, \leq, 0)$.
% is used instead of $\strC$.
%
%For every fixed set of clocks $\X$
%there are finitely many different constraints $\varphi(\bar x)$ up to logical equivalence.
%
Let $A = (\Sigma, L, \X, \Delta)$ be a \TA
and we build a fractional \TA $A' = (\Sigma', L', \X, \Delta')$
where $\Sigma'$ equals $\Sigma$
extended with an extra symbol $\tick \x \not\in\Sigma$ for every clock $\x \in \X$ of $A$,
and $L' = L \times \Lambda_M \times 2^\X \cup L_\bullet$,
where $\Lambda_M$ abstracts the integer value of clocks,
$2^\X$ keeps tracks of which clocks are \emph{not} allowed to be reset any more in the future,
and $L_\bullet$ contains some extra control locations used in the simulation.
%
Every transition $\trule p \op q \in \Delta$
generates one or more transitions in $\Delta'$
depending on $\op$. Assume that the initial control location of $A'$ is $\tuple {p, \lambda, \ZZ}$.
%
The simulation of $\readop a$ is immediate.
An operation $\testop \varphi$ is simulated by $\testop {\restrict \varphi \lambda}$,
%
%If $\op = \readop a$,
%then $\Delta'$ contains
%$\trule {\tuple {p, \lambda, \ZZ}} {\readop a} {\tuple{q, \lambda, \ZZ}}$,
%for every choice of $\lambda, \ZZ$.
%
%If $\op = \testop \varphi$,
%then $\Delta'$ contains
%$$\trule {\tuple {p, \lambda, \ZZ}} {\restrict \varphi \lambda} {\tuple{q, \lambda, \ZZ}},$$
where $\restrict \varphi \lambda$ is obtained by resolving all integer and modular constraints according to $\lambda$
(and thus contains only fractional constraints).
%
An operation $\op = \resetop \Y$
%then $\Delta'$ contains
%$$\trule {\tuple {p, \lambda, \ZZ}} {\resetop \Y} {\tuple{q, \lambda[\Y \mapsto 0], \ZZ \cup \ZZ_1}}$$
%
is only allowed if $\Y \subseteq \X \setminus \ZZ$ (no forbidden clocks are reset),
and it results in a new control location $\tuple{q, \lambda[\Y \mapsto 0], \ZZ \cup \ZZ_1}$
for every choice $\ZZ_1 \subseteq \Y$ of clocks which are declared to be reset now for the last time.
%
An operation $\op = \elapse$ is simulated by
updating the unary abstraction $\lambda$ for clocks that elapsed an integral amount of time
(this is done by checking whether their fractional part was wrapped around $0$);
additionally, for every clock $\x \in \ZZ$ that elapsed one time unit,
$A'$ reads one input letter $\tick \x$.
%
At the end of a time elapse transition
the control state is thus of the form $\tuple {q, \lambda', \ZZ}$.

\paragraph{Reconstruction of the reachability relation.}

We reconstruct the reachability relation of $A$ from that of $A'$ as follows.
%
For a set of words $L'$ of $A'$, let $\varphi_{L'}(y)$ be a formula with $\card \X$ free variables $y = (y_\x)_{\x \in \X}$
s.t.~variable $y_\x$ counts the number of $\tick \x$'s in words of $L'$.
%
For a set of clocks $\ZZ$ that is not reset
and for a set of words $L'$ of $A'$,
the relation between integral clocks of $A$ is reconstructed
according to the following formula
%
\begin{align*}
  \varphi_{\ZZ, L'}(\floor {\bar x}, \floor {\bar x'}) \equiv \varphi_{L'}(y),
\end{align*}
%
where, for every $\x \in \X$, $y_\x = \floor {\bar x'} - \floor {\bar x}$ if $x \in \ZZ$ and $y_\x = \floor {\bar x'}$ otherwise.
With these definitions in hand,
every atom $(L', \varphi')$ of the $\tuple {p,\lambda,\ZZ}, \tuple {q,\mu,\X}$-reachability relation of $A'$
(for some $\lambda,\ZZ,\mu$)
%is expressed by the semiatom
%
%$$\alpha_{\tuple {p,\lambda,\ZZ} \tuple {q,\mu,\X}} = (L_1', \varphi_1') + \cdots + (L_n', \varphi_n'),$$
%
%where, since $A'$ is fractional, the $\varphi_i(\fract{\bar x}, \fract{\bar x'})$'s
%denote the relation between initial $\fract{\bar x}$ and final $\fract{\bar x'}$ fractional clock values,
%then the $pq$-reachability relation of $A$ can be written as the semiatom
%
%\begin{align*}
%    \alpha_{pq} = \sum_{\lambda, \ZZ, \mu} (L_i, \varphi_i)
%\end{align*}
%
generates the atom $(L, \varphi)$ of the $pq$-reachability relation of $A$,
where $L$ is the projection of $L'$ to alphabet $\Sigma$, and
%
\begin{align*}
  \varphi(\floor {\bar x}, \fract{\bar x}, \floor {\bar x'}, \fract{\bar x'}) \equiv
    \varphi_\lambda(\floor {\bar x}) \wedge
    \varphi_{\ZZ, L'}(\floor {\bar x}, \floor {\bar x'}) \wedge
    \varphi'(\fract{\bar x}, \fract{\bar x'}) \wedge
    \varphi_\mu(\floor {\bar x'}).
\end{align*}

\subsection{Step 2: Fractional \TA}
\label{sec:fractional:TA}

In this section we compute the reachability relation for fractional \TA.
We make use of clock difference relations (\CDR) introduced in Sec.~\ref{sec:prelim:CDR}
to represent the relations between the fractional parts of initial and final clock values.
%
The base cases in the definition of reachability relation
are directly expressible by the following \emph{basic \CDR}:%
%\footnote{
%We write
%%$\fract {\x'} = \fract \x$ as a shorthand for $\fract {\x'-\x_0'} = \fract {\x-\x_0}$,
%$\fract {\x'} = 0$ as a shorthand for $\fract {\x'-\x_0'} = 0$.
%}:
%
\begin{align}
  \label{eq:CDR:read}
  \varphi_{\readop a} (\bar x, \bar x') &\equiv \varphi_{\id}(\bar x, \bar x'), \\
  \varphi_{\testop \psi} (\bar x, \bar x') &\equiv \varphi_{\id}(\bar x, \bar x') \wedge \tilde \psi(\bar x), \\
  \varphi_{\resetop \Y}(\bar x, \bar x') &\equiv
    \x_0' = \x_0 \wedge \bigwedge_{\x \in \Y} \fract {\x_0' - \x'} = \fract {\x_0'} \wedge
    \bigwedge_{\x \in \X \setminus \Y} \fract{\x_0' - \x'} = \fract {\x_0 - \x}, \textrm{ and } \\
  \label{eq:CDR:elapse}
  \varphi_{\elapse}(\bar x, \bar x') &\equiv
    \bigwedge_{\x \in \X} \fract{\x'_0 - \x'} = \fract{\x_0 - \x},
\end{align}
%
where $\tilde\psi$ is the \CDR logically equivalent to clock constraint $\psi$ obtained by \eqref{eq:CDR:zero}--\eqref{eq:CDR:leq}.
The following lemma states that the basic \CDR's above capture reachability for basic runs.
%
\begin{lemma}
  \label{lem:onestep:CDR}
  Let $p, q \in Q$, $\mu, \nu \in \Q^\X$, and $a \in \Sigma_\varepsilon$.
  %Let $\mu \reach a {pq} \nu$ be derived according to one of the basic cases \eqref{eq:reachrel:A}--\eqref{eq:reachrel:D}.
  Then, 
  \begin{align}
    \frac{}{\mu \reach a {pq} \nu}
    \qquad \textrm{ iff } \qquad
    \exists \tuple{p, \op, q} \in \Delta \st (\mu, \nu) \models \varphi_\op.
  \end{align}
\end{lemma}

%A fractional \TA transition $(p, \op, q)$ naturally induces a corresponding atom $\alpha$:
%if $\op = \resetop \Y, \elapse$, then $\alpha = (\set\varepsilon, \varphi_\op)$;
%if $\op = \testop \varphi$, then $\alpha = (\set\varepsilon, \varphi_\id \wedge \varphi)$;
%and if $\op = \readop a$, then $\alpha = (\set a, \varphi_\id)$.


%
%Concatenation
%$\sum_i a_i \;\cdot\; \sum_j b_j = \sum_{ij} a_i\cdot b_j$
%$\left(\sum_i a_i\right)^* = ...$
%
%Given a fractional and bounded \TA and two distinguished control locations $p, q$ therein,
%we can compute a semiatom denoting its ternary reachability relation.
%
\begin{theorem}
  The $pq$-reachability relation of a fractional \TA is expressible by a semiatom.
\end{theorem}

\begin{proof}
  We construct a modified finite reachability graph
  with configurations of the form $(r, \varphi)$
  with $r$ a control location and $\varphi$ a clock difference relation.
  %
  We start from $(p, \varphi_\id)$
  and whenever we have a rule $(r, \op, s)$ in the \TA
  and a configuration $(r, \varphi)$,
  we add a transition $(r, \varphi) \goesto a (s, \psi)$, where:
  if $\op = \resetop \Y, \elapse$, then $a=\varepsilon$ and $\psi \equiv \varphi \circ \varphi_\op$;
  if $\op = \testop \xi$, then $a=\varepsilon$ and $\psi \equiv \varphi \wedge \xi$;
  and if $\op = \readop b$, then $a = b$ and $\psi \equiv \varphi$.
  %
  We collect all reachable configurations of the form $(q, \varphi_1), \dots (q, \varphi_n)$,
  and for each of them we compute the (regular) set of words $L_i$
  s.t.~there exists a path from the initial configuration $(p, \varphi_\id)$ to $(q, \varphi_i)$.
  %
  The sought semiatom is then $(L_1, \varphi_1) + \cdots + (L_n, \varphi_n)$.
\end{proof}

